On Context Bisimulation for Parameterized Higher-order Processes

This paper studies context bisimulation for higher-order processes, in the presence of parameterization (viz. abstraction). We show that the extension of higher-order processes with process parameterization retains the characterization of context bisimulation by a much simpler form of bisimulation called normal bisimulation (viz. they are coincident), in which universal quantifiers are eliminated; whereas it is not the same with name parameterization. These results clarify further the bisimulation theory of higher-order processes, and also shed light on the essential distinction between the two kinds of parameterization.

==> eptcsdata.tex <==
\providecommand{\firstpage}{37}
\providecommand{\publicationstatus}{M. Carbone, I. Lanese, A. Lluch-Lafuente, A. Sokolova (Eds.):\\
6th Interaction and Concurrency Experience (ICE 2013)\\
EPTCS 131, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.131.5}{10.4204/EPTCS.131.5}}
\pdfoutput=1

